Affective Movement Generation using Laban Effort and Shape and Hidden Markov Models

Body movements are an important communication medium through which affective states can be discerned. Movements that convey affect can also give machines life-like attributes and help to create a more engaging human-machine interaction. This paper presents an approach for automatic affective movement generation that makes use of two movement abstractions: 1) Laban movement analysis (LMA), and 2) hidden Markov modeling. The LMA provides a systematic tool for an abstract representation of the kinematic and expressive characteristics of movements. Given a desired motion path on which a target emotion is to be overlaid, the proposed approach searches a labeled dataset in the LMA Effort and Shape space for similar movements to the desired motion path that convey the target emotion. An HMM abstraction of the identified movements is obtained and used with the desired motion path to generate a novel movement that is a modulated version of the desired motion path that conveys the target emotion. The extent of modulation can be varied, trading-off between kinematic and affective constraints in the generated movement. The proposed approach is tested using a full-body movement dataset. The efficacy of the proposed approach in generating movements with recognizable target emotions is assessed using a validated automatic recognition model and a user study. The target emotions were correctly recognized from the generated movements at a rate of 72% using the recognition model. Furthermore, participants in the user study were able to correctly perceive the target emotions from a sample of generated movements, although some cases of confusion were also observed.

==> abstract199.tex <==
This paper presents an approach for automatic affective movement generation that makes use of two movement abstractions:  1) Laban movement analysis, and 2) hidden Markov modeling. The Laban movement analysis provides a systematic tool for an abstract representation of the kinematic and expressive characteristics of movements.
Given a desired motion path on which a target emotion is to be overlaid, the proposed approach searches a labeled dataset in the Laban Effort and Shape space for movements similar to the desired motion path that convey the target emotion. An HMM abstraction of the identified movements is obtained and used with the desired motion path to generate a novel movement that is a modulated version of the desired motion path, conveying the target emotion. The extent of modulation can be varied, trading off between kinematic and affective constraints in the generated movement. The proposed approach is tested using a full-body movement dataset. The target emotions were correctly recognized from the generated movements at a rate of 72\% using a validated automatic recognition model. Furthermore, participants in a user study were able to correctly perceive the target emotions from a sample of generated movements, although some cases of confusion were also observed.


==> relatedFinal.tex <==
%related
In general, there are two main approaches for automatic affective movement generation: 1) rule-based, and 2) example-based. 
Rule-based approaches propose a set of motion generation/modification rules that are mainly driven by an intuitive mapping between movement features and different affective expressions (or motion styles).  On the other hand, example-based approaches generate a desired affective movement by concatenating or blending movement exemplars from a labeled dataset of movements. 

The success of rule-based approaches depends on a-priori knowledge of postural and motion cues salient to different affective expressions and how  these cues are incorporated into the rules in terms of quantitative variables that can be tuned to generate a desired affective movement. 
A drawback of the rule-based approaches is that they are designed for a specific  kinematic structure and a set of movements, and often are not readily adaptable to other structures and movements. While this limitation also exists for the example-based approaches, they do not rely on any deterministic rules and are capable of generating novel movement trajectories provided that adequate movement exemplars are available. Therefore, the success of the example-based approaches depends on the richness of the labeled  dataset.

Several examples of rule-based approaches can be found in the literature. A  mapping from Laban Effort and Shape to upper-body movement kinematics is proposed in \cite{Chi:2000}. Correlations between Laban components and discrete emotions  are used to devise a mapping from discrete emotions to joint angles of a humanoid robot \cite{Masuda2010}. In another study, a set of motion modification rules adjust the velocity, the range of motion, and the basic posture for a given movement based on specified levels of the arousal and valence affective dimensions \cite{Nakagawa2009}. A set of expressivity parameters  derived from the psychology literature (overall activation, spatial extent, temporal extent, fluidity, power, repetition) are used to develop rules that select a gesture type and modify it to adopt a desired style (e.g., abrupt) for an embodied conversational agent \cite{Hartmann2006}.

Example-based approaches range from concatenation of labeled motion segments (e.g., \cite{Arikan:2002}) to sophisticated generative models learned from exemplar movements (e.g., \cite{TaylorNIPS2006}).  Human movements vary in length and are intrinsically high-dimensional, and learning in high-dimensional motion space suffers from the limitations associated with the ``curse of dimensionality''.
 Different approaches are reported that make use of a low-dimensional  representation of affective movements along with an inverse mapping to generate new human movements. 
For instance, movements can be  represented as a weighted linear combination of a set of basis functions (functional representation) \cite{unuma1995fourier, SamadaniSocial2013}. The human gait is generated by interpolating or extrapolating Fourier expansions of actual human movements corresponding to different locomotion types (walk and run) subject to kinematic constraints (step size, speed, and hip position) \cite{unuma1995fourier}. Then, a gait is imbued with a target emotion via superposition of the Fourier expansion of the gait with a Fourier characteristic function for the target affective gait. 
In another study, a functional representation of a set of affective hand movements is obtained by transforming the movements into \textit{B}-spline basis space \cite{SamadaniSocial2013}. Then, functional principal component analysis is used to obtain a lower-dimensional subspace that serves as the basis space for affective movement generation. 
A limitation of the basis function expansion approaches is that they require movements to be of equal length with aligned landmarks, which is a difficult constraint to attain under natural conditions. 

Other example-based approaches learn a mapping between interpolation parameters and the human joint space to generate different motion trajectories. 
Mukai and Kuriyama \cite{Mukai:2005} employ a Gaussian process regression approach to learn such a mapping. For each action (e.g., arm reaching), a set of control parameters are manually selected (e.g., turning angle and height of the target for the reaching movement) and a mapping between the parameter space and high-dimensional joint space is learnt for that action. The resulting action-specific mapping is used to generate different styles of the action (e.g., reaching to different target positions).
Movement styles were annotated in terms of Laban Weight, Time, and Flow Effort for the movements available in a labeled dataset 
 \cite{Torresani2006NIPS}, and for each pair of kinematically similar movements, a new movement is generated 
  via space-time interpolation. Subsequently, a mapping between resulting motion styles and the interpolation parameters is learnt. For a test movement and a target style, a pair of movements in the labeled dataset are selected, whose blend is kinematically similar to the test movement and provides the best approximation of the target style \cite{Torresani2006NIPS}. The studies \cite{Mukai:2005,Torresani2006NIPS} do not explicitly address affective movement generation.  
   
Another class of example-based approaches derives a stochastic generative modeling of the movements. Among stochastic generative approaches, those that derive a  mapping from a lower-dimensional hidden space to the movement space are popular in human motion analysis. Style machines, a parametric hidden Markov modeling approach, provide a stochastic modeling of movements parametrized by a style variable to be used to generate movements with a desired style \cite{Brand:2000}.  Style machines were tested with a set of similar movements  performed in different styles (biped locomotion, and choreographed ballet dance), and were not explicitly tested to generate affective movements \cite{Brand:2000}. 
A Gaussian process (GP) dynamical model was used to learn motion styles as low-dimensional continuous latent variables and their mapping to movement observations. Using the learned model, a new movement is generated by adjusting the latent variable to adopt a desired style \cite{Wang2008}. GP-based models are often limited to a small number of aligned and similar movements, and 
are computationally expensive to learn, which hinders their application for large scale motion learning and generation. 
Taylor et al. \cite{TaylorNIPS2006} propose a parametric hierarchical modeling of human movements using conditional restricted Boltzmann machines (CRBM) for exact inference and generating stylistic human movements. Higher level layers representing high-level latent factors  can be sequentially added to the model as needed, to capture high-level structure in the movements, resulting in a deep belief network. 
In an extension to \cite{TaylorNIPS2006}, a set of context/style variables (discrete or continuous) is added to the CRBM to 
generate different motion styles, synthesize transitions between stylized motions as well as  interpolating and extrapolating the training data. However, learning CRBMs is challenging due the large number of parameters and metaparameters that need to be set \cite{HintonRBMGuide}.  
  

In this paper,  a new example-based affective movement generation approach is presented that aims to modulate a desired motion path to convey a target emotion.  The proposed approach exploits movements from the target emotion class that are kinematically 
similar  to the desired motion path  (nearest neighbours (NN)) 
 to generate a modulated version of the desired motion path that conveys the target emotion. The Laban Effort and Shape abstraction is used to identify the nearest neighbours. 
 The nearest neighbours along with the desired motion path are then encoded in an HMM and the most likely state sequence of the resulting HMM for the desired motion path is used to generate a modulated version of the desired motion path. 

